BANet: Bidirectional Aggregation Network with Occlusion Handling for Panoptic Segmentation

Panoptic segmentation aims to perform instance segmentation for foreground instances and semantic segmentation for background stuff simultaneously. The typical top-down pipeline concentrates on two key issues: 1) how to effectively model the intrinsic interaction between semantic segmentation and instance segmentation, and 2) how to properly handle occlusion for panoptic segmentation. Intuitively, the complementarity between semantic segmentation and instance segmentation can be leveraged to improve the performance. Besides, we notice that using detection/mask scores is insufficient for resolving the occlusion problem. Motivated by these observations, we propose a novel deep panoptic segmentation scheme based on a bidirectional learning pipeline. Moreover, we introduce a plug-and-play occlusion handling algorithm to deal with the occlusion between different object instances. The experimental results on COCO panoptic benchmark validate the effectiveness of our proposed method. Codes will be released soon at https://github.com/Mooonside/BANet.

==> sections/intro.tex <==
\section{Introduction}
% 	1. 任务定义
% 	2. 解决方案： top-down, bottom-up 其中top-down包含两个子任务和一个融合算法
% 	3. 两个子任务方面，介绍大家的工作，忽略了任务之间的互补性 not fully utilized
% 	4. 融合算法方面，介绍大家的工作，
%	5. In summary...
Panoptic segmentation, recently proposed by~\cite{kirillov2019panoptic1}, unifies semantic and instance segmentation. %Since this task was proposed, lots of efforts have been paid to solve it. 
%The prevalent approaches fall into two categories: top-down~\cite{Li2018Learning, xiong2019upsnet, li2019attention, liu2019end, xiong2019upsnet} and bottom-up~\cite{yang2019deeperlab}.
A typical paradigm for panotpic segmentation is of a top-down approach~\cite{Li2018Learning, xiong2019upsnet, li2019attention, liu2019end, xiong2019upsnet} in which instances are first identified and then assigned to semantic labels. %for the instance segmentation pipeline.
% The top-down methods use a proposal-based detector to find objects, while the bottom-up ones apply anchor-free detection through a fully convolutional network.  %todo: 说一下我们focus在top-down?
For top-down methods, there exist two key problems: 
\begin{inparaenum}[1)]
	\item how to improve semantic segmentation and instance segmentation coherently and
	\item how to combine results from instance segmentation and semantic segmentation into the final panoptic output.
\end{inparaenum}

It is observed that the complementarity between these two tasks could be utilized. For example, the object boundaries from instance segmentation can help semantic segmentation, while the contextual information in semantic segmentation can help instance segmentation.
Previous works~\cite{Li2018Learning, xiong2019upsnet, li2019attention} use score maps from instance segmentation to guide semantic segmentation. 
There lacks a path from semantic segmentation to instance segmentation. Besides, score maps alone are insufficient for information exchange due to the limited channel size.

To improve this, we design two lightweight modules, namely the instance-to-semantic~(I2S) and the semantic-to-instance~(S2I) module to build bidirectional paths for feature aggregation between these two tasks. Consequently, the original separate way of performing semantic and instance segmentation becomes interdependent and reciprocal. Specifically, S2I passes the context-abundant features from semantic segmentation to instance segmentation to help localization and recognition. Meanwhile, the instance-relevant features from instance segmentation are fed back to semantic segmentation to enhance resolution and context.


%To alleviate this issue, we propose two lightweight modules, namely the instance-to-semantic~(I2S) and the semantic-to-instance~(S2I) module. In order to exchange features between the two tasks, these two modules build a bidirectional path where features from instance head can be aligned and aggregated directly with features from semantic head with a new operation RoIInlay. 

%Another challenge lies in the occlusion among mask predictions. %To accomplish this, we need not only high-level category-relevant information, but also low-level appearance~(texture) as reference.
After performing semantic and instance segmentation, a fusion algorithm is needed to combine their results to the panoptic format. During this process, the belonging of occluded parts among objects must be determined. Previous works~\cite{kirillov2019panoptic1, liu2019end, de2018panoptic, xiong2019upsnet} based predictions on detection/mask scores. However, the order of scores is not always consistent with the actual spatial rank of objects. For example, a tie usually overlaps a person, but it tends to get lower score~(due to class imbalance). 

To alleviate this issue, we propose a learning-free texture-based fusion algorithm. It utilizes the similarity of low-level texture~(appearance), which is a strong visual cue for solving occlusion. Intuitively, if an object A overlaps B, the overlapped part should look more similar to A, rather than B. Motivated by this, our algorithm compares the similarity of texture between occluded parts and corresponding objects, and assign occluded parts to objects of closest texture. 

\begin{figure}[tb]
	\centering
	\begin{subfigure}{1.0 \linewidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figures/pipeline_a.pdf}
		\subcaption{
			\label{fig:Pipeline_a} 
		}
	\end{subfigure}%
	
	\begin{subfigure}{1.0\linewidth}
		\centering
		\includegraphics[width=1.0\linewidth]{figures/pipeline_b.pdf}
		\subcaption{
			\label{fig:Pipeline_b} 
		}
	\end{subfigure}%
\end{figure}



We summarize the contributions of our work as follows:
\begin{itemize}
	\item We design an end-to-end network for panoptic segmentation.
	\item We propose two novel modules, namely instance-to-semantic~(I2S) and semantic-to-instance~(S2I) to enable feature-level exchange between instance segmentation and semantic segmentation.
	\item We propose a learning-free texture-based fusion algorithm to better solve the occlusion among objects, which can be plugged in any top-down based networks.
\end{itemize}





%Holistic scene understanding is one of the most challenging problems in computer vision. Back to the pre-deep learning era, ~\cite{Tu2005Image} combined bottom-up and top-down methods to parse images into constituent visual patterns. However, the interst of holistic scene understanding faded in the deep-learning era due to lack of unified task definition and evaluation metrics. Researchers shifted focus to its subtasks: semantic segmentation, object detection and instances segmentation. 
%
%Thanks to the recently proposed Panoptic segmentation task \cite{kirillov2019panoptic1}, more and more attention are brought back to this task. Panoptic segmentation defines a standard output format and evaluation metric for it. Soon after its appearance, lots of efforts have been made. The initial attempts solve this task by combining results from a separate-trained semantic segmentation model and instance segmentation model~\cite{kirillov2019panoptic1}. Then, unified pipelines are proposed to use parallel heads based on a shared backbone for different tasks.

%researchers shifted focus to either semantic segmentation, or instances segmentation gradually. Until proposed the panoptic segmentation task.


==> sections/viz.tex <==
%\begin{figure*}
%	\centering
%\begin{subfigure}[b]{0.23\textwidth }
%		\begin{subfigure}[b]{1.0\textwidth }
%			\includegraphics[width=1.0\textwidth ]{figures/vis/ex_1.png}
%		\end{subfigure}
%	
%		\begin{subfigure}[b]{1.0\textwidth }
%			\includegraphics[width=1.0\textwidth ]{figures/vis/ex_2.png}
%		\end{subfigure}
%	
%		\begin{subfigure}[b]{1.0\textwidth}
%			\includegraphics[width=1.0\textwidth ]{figures/vis/ex_3.png}
%		\end{subfigure}
%		\begin{subfigure}[b]{1.0\textwidth }
%			\includegraphics[width=1.0\textwidth ]{figures/vis/ex_4.png}
%		\end{subfigure}
%		\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/ex_4.png}
%	\end{subfigure}
%		\begin{subfigure}[b]{1.0\textwidth }
%	\includegraphics[width=1.0\textwidth ]{figures/vis/ex_4.png}
%\end{subfigure}
%		\caption{Image}
%\end{subfigure}
%	\hspace{1pt}
%\begin{subfigure}[b]{0.23\textwidth }
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_1.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_2.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_3.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_4.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_4.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/gt_4.png}
%	\end{subfigure}
%	\caption{Ground Truth}
%\end{subfigure}
%\hspace{1pt}
%\begin{subfigure}[b]{0.23\textwidth }
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_1.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_2.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_3.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_4.png}
%	\end{subfigure}
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_4.png}
%	\end{subfigure}
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/bl_4.png}
%	\end{subfigure}
%	\caption{Baseline}
%\end{subfigure}
%	\hspace{1pt}
%\begin{subfigure}[b]{0.23\textwidth }
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_1.png}
%	\end{subfigure}
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_2.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_3.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_4.png}
%	\end{subfigure}
%
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_4.png}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{1.0\textwidth }
%		\includegraphics[width=1.0\textwidth ]{figures/vis/oh_4.png}
%	\end{subfigure}
%	\caption{Our Model}
%\end{subfigure}
%	\caption{Visualization}\label{fig:visual}
%\end{figure*}
